Cloud Deployment Tradeoffs for the Analysis of Spatially-Distributed Systems of Internet-of-Things

Internet-enabled things and devices operating in the physical world are increasingly integrated in modern distributed systems, supporting functionalities that require assurances that certain critical requirements are satisfied by the overall system. We focus here on spatially-distributed Internet-of-Things systems such as smart environments, where the dynamics of spatial distribution of entities in the system is crucial to requirements satisfaction. Analysis techniques need to be in place while systems operate to ensure that requirements are fulfilled. This may be achieved by keeping a model of the system at runtime, monitoring events that lead to changes in the spatial environment, and performing analysis. This computationally-intensive runtime assurance method cannot be supported by resource-constrained devices that populate the space and must be offloaded to the cloud. However, challenges arise regarding resource allocation and cost, especially when the workload is unknown at the system's design time. As such, it may be difficult or even impossible to guarantee application service level agreements, e.g., on response times. To this end, we instantiate spatial verification processes, integrating them to the service layer of an IoT-cloud architecture based on microservices. We propose several cloud deployments for such an architecture for assurance of spatial requirements -- based on virtual machines, containers, and the recent Functions-as-a-Service paradigm. Then, we assess deployments' tradeoffs in terms of elasticity, performance and cost by using a workload scenario from a known dataset of taxis roaming in Beijing. We argue that the approach can be replicated in the design process of similar kinds of spatially distributed Internet-of-Things systems.

==> sections/iot-architecture.tex <==
%!TEX root = ../paper.tex

% \section{Microservices for Internet-of-Things}
% \section{Spatial Analysis at Runtime for the Internet-of-Things}

\section{Motivating example: Bike-Sharing in a Smart City}
\label{sec:motivation-example}

In this section, we introduce a motivating scenario serving as a running example of an exemplar spatially-distributed internet-of-things system throughout the paper. We begin with a brief description of the scenario's setting and then consider SLA goals that the system should exhibit as well as the challenges that arise to do so. 
% Subsequently, we illustrate how such goals and challenges can be addressed through a generic service-based cloud architecture as a solution for performing spatial analysis.   

% \christos{propose title: Microservices for the internet-of-things}
% \martin{I agree with the title but we should be careful to explain (here or in the introduction/paper outline) what is this section about}
% \christos{I have been thinking, about the way we structured the paper. Should we remove "as microservices" from the paper title? then in this section, we describe overall setting. Then in section 6, we show different cloud architectures that can support the problem setting, focusing a bit more on microservices which we argue provide the most elegant, low-maintenance etc solution. In the evaluation, we compare, and in the conclusions we say that we showed that microservices perform better but..etc. what do you think? }
% \christos{title could even be: Spatial Model Checking at Runtime for the Cloud-enabled Internet-of-Things?}
%\begin{itemize}
%	\item maybe example should be in this section, and remove architecture from the title (Arch will be later)
%	\item high level architecture picture but discuss deployment, mention mobile devices, global state
%	\item high level explanation of how it works
%	\item emphasis on IoT, novelty 
%	\item explain over the example - bikes are moving inside the graph! other things may be inside, mention the WSN case
%\end{itemize}


\input{sections/example}


Challenges inherent in the motivating scenario considered include both evaluating the truth values of sub-goals (G1) and (G2) for all bikes in the city at any moment, as well as architecturally supporting this analysis. 
Notice how the evaluation of sub-goals for each bike depends on the position of all other bikes in the city -- the system's global state-- rendering the sub-goals \emph{global spatial properties}~\cite{fse17}. Additionally, evaluation of such global properties is challenging because of computational and scalability concerns, requiring a dedicated architecture for the overall IoT system. 
% \subsection{Computation at the device}
A na{\"i}ve approach would be to perform computation upon the devices constituting the IoT system themselves. In this case, the advantages are reduced latency and minimal persistent connectivity needs, as long as devices support the computation workload. However, the main disadvantage of this approach is the severe limitation on the computing resources of the IoT devices~\cite{song17offloading}. Even considering a top-of-the-range smartphone or tablet, SLA constraints and prohibitive battery drain make this approach unfeasible in practice~\cite{GarrigaMendonca2017} (see also Section~\ref{sec:evaluation}). %Nevertheless,  presents the evaluation of this alternative, where performing computation at the device proves to be prohibitively time-consuming. 

%\subsection{Challenges for Cloud Deployment (new stuff)}

%Heavy computational workload
%Environment - Special circumstances (challenges).
%Computation intensive. No memory/data restrictions.
% \martin{beginning of the new part regarding cloud offloading challenges}




































% %A critical requirement of an IoT is that the things in the network must be interconnected. 
% IoT system architectures bridge the gap between the physical and the virtual worlds, but entail multiple challenging factors. Design of IoT architecture involves networking, communication, extensibility, scalability, and interoperability among heterogeneous devices~\cite{li2015internet}. These devices may be heavily resource-constrained, e.g., in terms of computational power and battery (See Section~\ref{sec:evaluation}), and at the same time IoT applications have stringent quality of-service requirements, hindering the provision of computing and communication supports~\cite{Yu18infocom}. 

% Due to the fact that things may move geographically and need to interact with others in real-time mode,such an architecture should be adaptive, and support technology-agnostic communication of events. In addition, IoT should possess the decentralized and heterogeneous nature. 

% In this context, Service-Oriented Architectures (SOA) ensures the interoperability among the heterogeneous devices in multiple ways~\cite{li2015internet}, and allows to treat such a complex system as a set of well-defined simple services~\cite{baresi2017microservices}. In our approach, IoT services are indeed microservices~\cite{lewis14microservices,garriga2017towards}, as they are small, modular, communicate with lightweight mechanisms (often through an HTTP RESTful API) and are independently deployable by fully automated machinery.


% Those IoT microservices consist of a set of artifacts that fulfill a given functionality. We propose a service model in which stateless components (i.e., the model checker algorithm) and mostly immutable data (i.e., the topological graph of space) form \textit{stateless microservices}; analogously, stateful components (i.e., the global state defined as the current position of all the things) form \textit{stateful microservices}. In this manner, those microservices can be reused, scaled and maintained individually; therefore, the software and hardware components in an IoT deployment can be reused and upgraded efficiently. 

% Due to these advantages, SoA has been widely applied as a mainstream architecture,  for example in the context of Wireless Sensors Networks (WSNs). SOA applied to IoT provides extensibility, scalability, modularity and interoperability among heterogeneous things; in addition, the functionalities and capabilities are abstracted into a common set of services.


% Figure~\ref{fig:iot-arch} provides a generic SoA view for IoT in the context of our problem, which consists of three layers~\cite{li2015internet}:


% \begin{itemize}
% 	\item Sensing/Actuating layer is integrated with available devices/things to sense their status and act upon some decision based on that status.
% 	\item Network layer is the infrastructure that supports wireless or wired connection among things.
% 	\item Microservice layer creates and manage services required by users or applications.
% \end{itemize}

% Back to our running example, a bike's location sensors (sensing layer) emit heartbeats with its coordinates, either periodically or upon certain events (e.g. locking/unlocking). Those heartbeats should trigger the evaluation of the model in order to determine whether the defined sub-goals hold for the current position of the bike. 

% The event travels across a WSN, or the Cellular Network towards the Cloud (Network layer), reaching the microservices in charge of processing it (Service Layer). The API Gateway receives the event and forwards it to the corresponding microservices: the state keeper microservice (in charge of keeping the current, dynamic state of the system) and the checker microservice (in charge of evaluating the sub-goal for the bike associated to the event). 

% Finally, the result of the evaluation travels back from the microservices to the actuator layer, to undertake the corresponding actions through the mobile device of the user (e.g., providing feedback regarding penalties/rewards) or the bike itself (i.e., locking/unlocking).

  
% \begin{figure*}[htbp]
% 	\centering
% 	\includegraphics[width=1\textwidth]{img/iot-arch-draft}
% 	\caption{Microservices Architecture for IoT [DRAFT]\martin{change for definitive}.}
% 	\label{fig:iot-arch}
% \end{figure*}
